Generating Critical Scenarios for Testing Automated Driving Systems

Autonomous vehicles (AVs) have demonstrated significant potential in revolutionizing transportation, yet ensuring their safety and reliability remains a critical challenge, especially when exposed to dynamic and unpredictable environments. Real-world testing of an Autonomous Driving System (ADS) is both expensive and risky, making simulation-based testing a preferred approach. In this paper, we propose AVASTRA, a Reinforcement Learning (RL)-based approach to generate realistic critical scenarios for testing ADSs in simulation environments. To capture the complexity of driving scenarios, AVASTRA comprehensively represents the environment by both the internal states of an ADS under-test (e.g., the status of the ADS's core components, speed, or acceleration) and the external states of the surrounding factors in the simulation environment (e.g., weather, traffic flow, or road condition). AVASTRA trains the RL agent to effectively configure the simulation environment that places the AV in dangerous situations and potentially leads it to collisions. We introduce a diverse set of actions that allows the RL agent to systematically configure both environmental conditions and traffic participants. Additionally, based on established safety requirements, we enforce heuristic constraints to ensure the realism and relevance of the generated test scenarios. AVASTRA is evaluated on two popular simulation maps with four different road configurations. Our results show AVASTRA's ability to outperform the state-of-the-art approach by generating 30% to 115% more collision scenarios. Compared to the baseline based on Random Search, AVASTRA achieves up to 275% better performance. These results highlight the effectiveness of AVASTRA in enhancing the safety testing of AVs through realistic comprehensive critical scenario generation.

==> 10.behavior_modeling.tex <==
\section{Behavior Modeling}

In this section, we model 4 basic driving behaviors, namely Acceleration, Steady Driving, Deceleration and dir Changing. Then, we define and formulate some specific behaviors that are combinations of these basic ones. 

\subsection{Basic Behavior Modeling}





\subsection{Specific Behavior Modeling}

\subsubsection{Lane Changing}

\subsubsection{Turning}


\subsubsection{Backing}

\subsubsection{Passing}


\subsubsection{Cruising}


\subsubsection{Stopping}


==> 2.background.tex <==
\section{Background}
\subsection{Automated Driving System}
\subsection{Simulation-based Testing}
\subsection{Reinforcement Learning}

==> 2.violation_modeling.tex <==
\section{Safety Condition Modeling}

\input{violations/general}
\input{violations/acceleration}
\input{violations/deceleration}
\input{violations/turn}
\input{violations/lane_changing}
\input{violations/overtaking}








==> 2.violation_modeling_backup.tex <==
\section{Safety violation modeling}
\label{violation-modeling}

% \subsection{Distance-Based Violations}
% Despite the existence of numerous traffic regulations, a vast majority are clearly defined and can be directly enforced through rule implementation during the development of autonomous vehicles. However, several regulations, such as those concerning general principles of speed and distance while driving, exhibit a degree of ambiguity. These ambiguous regulations are characterized by their contextual relevance and limitations that vary dynamically based on specific traffic conditions. Consequently, our research primarily focuses on these ambiguous regulations. Based on real-world traffic tickets, we models the following seven distance-based violations relating to the basic behaviours of AVs (cruising, stopping, lane changing) as defined in the Apollo system:

% \begin{itemize}
%     \item Improper turning: Occurs when a turn is made without adequately considering the surrounding traffic.
%     \item Improper lane changing: Happens when switching lanes without proper attention to nearby vehicles.
%     \item Improper passing: Involves attempting to overtake another vehicle in an unsafe manner.
%     \item Sudden braking: Entails abruptly applying the brakes without maintaining a safe distance from the vehicle behind, significantly increasing the risk of rear-end collisions.
%     \item Dangerous speeding: Involves driving at a speed unsuitable for the current traffic conditions, which can drastically reduce the reaction time needed to keep safe distances between vehicles.
%     \item Running a red light: Involves entering an intersection when the traffic signal is red or stopping beyond the designated stop line.
%     \item Collision: This violation represents the ultimate consequence of failing to maintain safe distances and following traffic regulations. It can involve any type of collision with another obstacles (e.g., vehicle, pedestrian).
% \end{itemize}

% All of the aforementioned violations share a common factor: they relate to the maintenance of safe distances by AVs from other vehicles while participating in traffic. To determine whether an AV is committing one of these violations, we first identify the specific behaviour the AV is performing and then determine if a violation is occurring.
% % \begin{itemize}
% %     \item Initiation Conditions
% %     \begin{itemize}
% %         \item Turning and Lane Changing: We utilize the vehicle’s heading, waypoint coordinates, and lane ID. If the vehicle tends to change its heading, and the upcoming waypoints belong to a different lane while the new direction remains parallel to the previous one, it is considered a lane change. Similarly, if the new direction forms a larger angle with the previous one, it indicates turning.
% %         \item Passing: This behavior occurs when an NPC vehicle changes and ego vehicle are moving in the same direction. The distance between the two vehicles gradually decreases during this maneuver. Specifically, the ego vehicle transitions from being behind the NPC vehicle to moving ahead of it within different lanes.
% %         \item Braking: Sudden braking occurs when the ego vehicle’s braking intensity abruptly increases while in motion.
% %         \item Accelerating: This situation involves high speeds and acceleration.
% %         \item Cruising: When encountering traffic lights (in red) or stop signs, or when pedestrians are present.
% %     \end{itemize}


Because \tool's main objective is to generate dangerous violations with a high risk of causing serious collisions, we will focus on examining interactions between autonomous vehicles and other vehicles that meet the following prerequisites:

\begin{center}
    $isIntersect = ((P_{ego} \leq \tilde{P}_{I} \leq \tilde{P}_{ego}) \vee  (P_{ego} \geq \tilde{P}_{I} \geq \tilde{P}_{ego})) \wedge ((P_{npc} \leq \tilde{P}_{I} \leq \tilde{P}_{npc}) \vee (P_{npc} \geq \tilde{P}_{I} \geq \tilde{P}_{npc}))$
\end{center}


The first task is to determine which behavior the AV is performing (e.g., turning, passing, etc.). To enhance the clarity and intuitiveness of behavior identification, we utilize a diverse set of variables. These variables provide a straightforward means of defining the conditions under which specific behaviors emerge. Given the extensive range of variables involved, we have systematically categorized them into two main types to streamline analysis and interpretation.

\textbf{\textit{Driving status. }}The variables in this category describe the position, movement status, and direction of the objects. These variables are detailed comprehensively in Table~\ref{tab:driving-status} .



\textbf{\textit{Road status.}} The variables in this category describe the lane, traffic light and predicted point. These variables are detailed comprehensively in Table \ref{tab:road-status}



Using the aforementioned variables, we define the conditions under which violations occur as follows:

\subsection{Sudden braking}
Sudden braking involves abruptly applying the brakes without maintaining a safe distance from the vehicle behind, thereby significantly increasing the risk of rear-end collisions. The braking behavior can be identified by the condition:

\begin{center}
  $isBraking = brake_{ego} > 0$    
\end{center}

Then, a braking action will be consideređ as a violation when:
% \vspace{0.5cm}
%         \begin{center}
%             $( brake_{ego} - brake^{past}_{ego}) > \theta_{brake}$ 
%         \end{center}
% \vspace{0.5cm}

% \begin{center}
%     \(isSuddenBraking = isBraking \, \text{ \& } \,  (brake_{ego} - brake^{past}_{ego} > \theta_{brake}) \, \text{ \& } \, (vioRate = 1) \text{ \& } isIntersect\)
% \end{center}

\begin{center}
    \(isSuddenBraking = \text{True if}  
    \begin{cases} 
        isBraking \\
        (brake_{ego} - brake^{past}_{ego} > \theta_{brake}) \\
        vioRate = 1 \\
        isIntersect
    \end{cases}\)
    % isBraking \, \text{ \& } \,  (brake_{ego} - brake^{past}_{ego} > \theta_{brake}) \, \text{ \& } \, (vioRate = 1) \text{ \& } isIntersect\)
\end{center}


% \begin{center}
%     \(isSuddenBraking = \text{True if}  
%     \begin{cases} 
%         brake_{ego} - brake^{past}_{ego} > \theta_{brake} \\
%         isBraking \\ 
%         vioRate = 1
%     \end{cases}\)
% \end{center}


\subsection{Dangerous speeding}
Dangerous speeding involves an autonomous vehicle moving at high speed and potentially crashing into other vehicles in front of it. In reality, this would be one of the common scenarios that could cause significant damage.
The speeding behavior can be identified by the condition: 
\begin{center}
$ isSpeeding = (v_{ego} > \theta_{speed}) \, \wedge  \, (a_{ego} > 0) $    
\end{center}

Then, a speeding action will be considered as a violation when:

\begin{center}
    \(isDangerousSpeeding = \text{True if}  
    \begin{cases} 
        isSpeeding \\
        vioRate = 1 \\
        isIntersect
    \end{cases}\)
\end{center}

\subsection{Improper passing}

For the case of "Improper Passing," these violations refer to situations where an autonomous vehicle intends to move ahead of another vehicle. In this scenario, the ego vehicle is behind, traveling at a higher speed compared to the other vehicle, and continues to accelerate. The conditions leading to this violation can be summarized as follows:

\begin{center}
$ isPassing = (\overrightarrow{v_{ego}} \cdot \overrightarrow{v_{npc}} > 0) \, \wedge \, (v_{ego} > v_{ego}) \, \wedge \, (a_{ego} > 0 ) \, \wedge \, (\overrightarrow{v_{ego}} \cdot (P_{ego} - P_{npc}) < 0)$    
\end{center}

When passing maneuvers bring vehicles very close together and their trajectories remain directed towards each other, it implies a high risk of collision. In such cases, the passing action would indeed constitute a violation.


\begin{center}
    \(isImproperPassing = \text{True if}  
    \begin{cases} 
        isPassing \\
        vioRate = 1 \\
        isIntersect
    \end{cases}\)
\end{center}


\subsection{Improper lane changing}
Changing direction while moving is one of the most fundamental and common behaviors, yet it also carries a significant risk of causing serious collisions. Improper lane changing is indeed one of such violations, occurring when a vehicle intends to move into an adjacent lane. In this context, one critical factor to consider is the angle deviation between the autonomous vehicle and its current lane, as well as the lane direction in the future. So the formula for this behavior is as follows:

\begin{center}
$ isLaneChanging = (\,( \overrightarrow{v\vphantom{d}_{ego}} , \overrightarrow{d_{lane}}) > \theta_{lc}) \wedge (\overrightarrow{d_{lane}} \parallel \overrightarrow{d_{\widetilde{lane}}} )$    
\end{center}

When performing a lane change, an autonomous vehicle will violate if it enters the safe distance of a vehicle traveling in the adjacent lane. In other words, the distance between them is not ensured. So, this violation is identified by following condition:

\begin{center}
    \(isImproperLC = \text{True if}  
    \begin{cases} 
        isLaneChanging \\
        vioRate = 1 \\
        isIntersect
    \end{cases}\)
\end{center}

\subsection{Improper turning}

Similarly to improper lane changing, improper turning also involves violations related to the vehicle's changing driving direction behavior. However, the key difference lies in the larger required turning angle and the future lane direction not necessarily being parallel to the current lane. Therefore, the conditions defining this behavior are as follows:

\begin{center}
$ isTurning = (\,( \overrightarrow{v\vphantom{d}_{ego}} , \overrightarrow{d_{lane}}) > \theta_{turning}) \wedge (\overrightarrow{d_{lane}} \nparallel \overrightarrow{d_{\widetilde{lane}}} )$    
\end{center}

Following that, if the autonomous vehicle continues to turn despite having an obstacle very close by, it constitutes a case of improper turning. This case is represented by following formula:

\begin{center}
    \(isImproperTurning = \text{True if}  
    \begin{cases} 
        isTurning \\
        vioRate = 1 \\
        isIntersect
    \end{cases}\)
\end{center}

\subsection{Run on a red light}

Involves entering an intersection when the traffic signal is red or stopping beyond the designated stop line.

\begin{center}
    $isRunOnRedLight = \text{True if} 
    \begin{cases}
    light_{status} = RED \\
    stop\_line(P_{ego}) \times stop\_line(P^{past}_{ego}) < 0
    
    \end{cases}
    $
    
\end{center}


% All of the aforementioned violations share a common factor: they relate to the maintenance of safe distances by AVs from other vehicles while participating in traffic. To determine whether an AV is committing one of these violations, we first identify the specific behaviour the AV is performing and then determine if a violation is occurring.

\subsection{Violation Severity Calculation}
    MoViTe uses a metric called Violation Rate (VioRate) to assess the level of violations by AV. The value of VioRate is directly proportional to the proximity of AV violations. This metric is determined based on the ‘Safety Distance’ and the ‘Current Distance’ between AV and other vehicles.
\subsubsection{Safety Distance}
    Safety Distance is a commonly used physical quantity in various AV quality assurance research. It is defined as the minimum distance an AV must maintain from another object to avoid collisions, even in the worst-case scenario. Related studies typically use two types of Safety Distance: \textit{Longitudinal Safety Distance} (LoSD) and \textit{Lateral Safety Distance} (LaSD). While LoSD facilitates calculations for objects moving in the same lane as the AV, LaSD is applied to objects in adjacent lanes. However, real-world traffic scenarios present a more complex challenge. AVs frequently encounter vehicles in non-adjacent lanes, particularly when entering intersections. In these situations, LoSD and LaSD are inadequate to provide a complete picture of the necessary Safety Distance for all surrounding objects.
    
    To address this issue, we propose not considering the relative position of the AV with respect to the lanes. Instead, we will use a two-dimensional coordinate system and determine the projections of surrounding objects onto the X and Y axes. Specifically, we will utilize the UTM coordinate system used in LGSVL to represent positional points and velocity values. Although UTM is inherently a three-dimensional coordinate system, we will simplify it to two dimensions by excluding the height axis, as height values of objects typically exhibit minimal variation over short road segments.
    
    By projecting the velocity vectors of the AV and other objects onto the Easting and Northing axes, we can treat each vehicle as two moving objects, one for each axis. Consequently, for any two vehicles, we calculate the Safety Distance along the Easting axis (EaSD) and the Safety Distance along the Northing axis (NoSD) based on their projections. Since projections on the same axis will move as if on a single-lane road, we employ two formulas to calculate the EaSD and NoSD for scenarios where the projections move in same direction and when they move in the opposite direction.
    
    \vspace{0.5cm}
    \textbf{\textit{Same direction:}}
    \begin{center}
        $d_{min,sa} = v_{f}*\tau + \frac{1}{2}( \frac{v_f^2}{\alpha_{f}} - \frac{v_l^2}{\alpha_{l}})$
    \end{center}

    \textbf{\textit{Opposite direction:}}
    \begin{center}
        $d_{min,op} = ( v_{1} + v_{2})*\tau + \frac{1}{2}( \frac{v_1^2}{\alpha_{1}} + \frac{v_2^2}{\alpha_{2}})$
    \end{center}
 \vspace{0.5cm}
    

    
\subsubsection{Violation Rate}
    Excluding violations related to traffic signs, we compute the violation severity based on the Safety Distance (SD) and Current Distance (CD) between the ego vehicle and other vehicles within its vicinity.
    The violation rate (VioRate) is defined as follows:
\begin{center}
    \(VioRate = 
    \begin{cases} 
        \displaystyle{\frac{SD}{CD}}, & \text{} CD > SD \\
        1.0, & \text{else}
    \end{cases}\)
\end{center}
        However, since SD does not account for the orientation of vehicles, there are cases where (VioRate = 1) but it may not truly represent a violation (e.g., Passing scenario with both vehicles maintaining parallel headings). To address this, we introduce an intersection point based on the current trajectory (determined by the vehicle’s position and velocity vector). If the paths of the ego vehicle and NPCs intersect behind either vehicle or do not intersect at all, their impact on each other is minimal, and we multiply (VioRate) by 0.5 in such cases.
        For the violation related to Running a Red Light or Stop Sign, we calculate (CD) as the distance from the vehicle to the stopping line. We use a sigmoid function to express the violation severity:
\begin{center}
    \(SignVio = 
    \begin{cases} 
       2 \left(1 - \frac{1}{1 + e^{-CD}}\right), & \text{if the vehicle stops before the line}  \\
        1.0, & \text{else}
    \end{cases}\)
\end{center}



==> 3.1.relistic_collisions.tex <==
\section{The Realism of the Generated Scenarios}

In this work, we propose several heuristic constraints to guarantee the realism of the generated scenarios. In practice, only focusing on the number of collisions occurred in the generated scenarios, various unrealistic scenarios could be generated. Such scenarios lead to waste time and resources on debugging yet do not bring any actual benefits. Therefore, \tool introduces several constraints to prevent the agent from selecting actions.


\textbf{Distance constraint.}

\textbf{Position constraint.}

\textbf{Speed constraint.}



==> 3.approach_backup.tex <==
\section{Safety violation scenario generation}

% This section describes our approach for generating challenging and diverse safety violation scenarios. Figure \ref{} illustrates overview of \tool.

% \begin{itemize}
%     \item Overview architecture of \tool
% \end{itemize}

% \tool models the problem as a MDP (Markov Decision Process) and then takes advantage of Reinforcement Learning algorithms to address. Specifically, we holistically consider the properties of the external environment and automated vehicle (AV) internal system to use as states. Actions are operations that change the environment's states, and we focus on actions related to vehicle behaviors because of their potential in causing violation. Reward is calculated in Multi-objective form, based on Violation rate and Diversity of each scenario.

% \subsection{Problem Modeling}

% The operating environment of AV is extremely complex and constantly changing, both in term of the external environment and the vehicle's internal systems. The reason is that the environmen is composed of many elements, including static objects (ie. traffic lights, signs), dynamic objects (ie. pedestrians, vehicles) and components of the vehicle's internal system (ie. Perception, Prediction). These factors also change continuously, such as the weather can transition from sunny to rainy, or the AV's internal parameters can vary within a wide range of values over time. As a result, generalizing the operating environment of AV, as well as learning and adapting from it, is a real challenge for AV-related researchers.

% Reinforcement Learning (RL) will be a good solution for the above problem. Instead of using a fixed ground truth as other Supervised Learning Algorithms, RL gives reward for each behavior implemented by Agent to evaluate their effectiveness. As the time goes on, RL operates and evaluates almost environment behaviors, even when it is continuously changing. Simultaneously, agent learns the way to choose appropriate actions to maximize the reward received at each time. Leveraging that flexible learning ability, \tool model the problem into an Markov Decision Process (MDP), and use the RL algorithm to solve. 

% The operating environment contains both the vehicle's internal system and its surrounding environment. To be able to generalize that environment, \tool takes advantage of information related to the external environment (ie. time, weather, traffic light) and the vehicle's internal system (ie. Perception, Prediction). Actions are operations that change the state of the environment, for example, changing from rain to fog, morning to noon, or adding vehicles to the testing environment. Reward will be calculated in a multi-objective manner, which represents the probability of each type of violation and diversity of current scenario. Besides, we apply a continuous weight adjustment method to balance the occurrence frequency of violations. For the reinforcement learning network, we take advantage of two algorithms, DDQN and PER, to minimize overestimation and expand the range of actions to be executed, thereby making the scenarios more diverse and realistic.

% \subsection{Holistic State Consideration:}

% The first task in \tool is to describe the AV's operating environment to help RL's Agent understand. Thus, we employee both external and internal states to generalize the characteristics of the operating environment. These are two fundamental aspects that directly affect the vehicle's performance and the violation probability of a scenario. They complement each other and combine together to bring out the most detailed informations of the environment. Thereby helping the model to adapt and accurately assess the environment at each time.

% \subsubsection{External States}

% External state refers to information obtained from the AV's surrounding environment. Those features include weather conditions (rain, fog, humidity), time (morning, noon, afternoon) and traffic light status. These information are considered the most basic,  having a direct impact on the ability to operate and make decisions of automated vehicle (bad weather can affect the ability of sensors to operate). In addition, after consulting a study on the impact of external attributes on a collision scenario, we decided to take advantage the following 6 additional attributes to generalize our current scenario, including:

% \begin{itemize}
%     \item Number of obstacles (\textbf{obs\_num}): Calculated by the total number of static and dynamic objects surrounding the AV. Having many obstalces around, AV might encounter more potential violations and could be affected in handling ability.  
%     \item Number of vehicles (\textbf{veh\_num}): This state is calculated in the same way to \textbf{obs\_num}, but only focuses on vehicles. The reason is that vehicles are among the most hazardous factors, posing the highest risks of accidents.
%     \item Distance to the nearest obstacle (\textbf{dis\_to\_nearest}): The smaller the distance between the subject and surrounding moving objects, the more accurately the vehicle has to handle to assure its safety. So this feature could show the danger level of environment.
%     \item Velocity of the nearest obstacle (\textbf{vel\_of\_nearest}): Besides distance, speed is information we use to describe the nearest object, providing a better representation of the environmental conditions.
%     \item Volume of the nearest obstalce (\textbf{vol\_of\_nearest}): Volume has the same role as speed, also provides more information about this obstalce.
%     \item Distance to the fastest obstacle (\textbf{dis\_to\_fastest}): In many scenarios, the subject commits a traffic violation due to not promptly avoiding vehicles approaching at high speed from afar. Therefore, this is also a potential state in causing violations.
% \end{itemize}

% All of the above mentioned attributes generalize the vehicle's external environment. Maybe when considering only one single attribute, they could not have much impact on the vehicle's ability to commit traffic violations. However, when combined together (e.g. a scenario where the number of vehicles is large and the distance to the fastest object is small, the vehicle will be placed in a more dangerous situation), all of these attributes will show the danger level of external factors.

% \subsubsection{Internal States}

% Besides external states, we also comprehensively consider the internal attributes of the automated vehicle system. These internal attributes can be understood as the characteristics that reflect the operational state of each component within the vehicle. Since entering real-world testing, there have been reports of over 500 traffic accidents involving automated vehicles. The primary cause of these incidents is inaccuracies in the operation of components within the vehicle system, such as inadequate detection of objects in front of the vehicle and incorrect decision-making. Therefore, the internal factors of the vehicle will greatly impact its traffic violation potential and will be useful in generating test scenarios.

% Treating automated vehicles like humans, we will leverage the information from the vehicle based on its modules, including Localization, Perception, Prediction and Planning \& Control. However, the states obtained from the vehicle system is subjective and may not always be accurate in many cases. As a result, we will utilize data obtained from simulations to verify the accuracy of the information from the vehicle system.

% \vspace{0.25cm}
% \noindent\textbf{Localization-related states}
% \vspace{0.25cm}

% Localization is one of the most crucial modules, tasked with determining the vehicle's position and providing supplementary information for various other modules. According to our observations, there are numerous instances where discrepancies arise between the position reported by the Localization module and the actual position. For example, we observed a situation with a significant discrepancy, approximately 5 meters along the x-axis and 17 meters along the y-axis. This represents a relatively large deviation, and in reality, the likelihood of violations occurring in this state could be quite high.

% Therefore, we have decided to utilize states to demonstrate the accuracy of the localization process. The first state is the discrepancy distance between the actual position and the localized position. This distance is denoted as D, with the following formula:


% \begin{center}
%     $D = \sqrt{(x_{local} - x_{real})^2 + (y_{local} - y_{real})^2}$
% \end{center}

% Where $x_{local}, y_{local}$ are the coordinates obtained from the vehicle system, while $x_{real}, y_{real}$ are the actual coordinates. The distance D can already indicate the degree of deviation through its magnitude. However, in many situations, the angle deviation between these two positions also has a significant impact. For example, in the case of a vehicle stopping at a red light, a misalignment of the localized position to the rear can lead to other modules making decisions to move forward, potentially resulting in a violation. Therefore, we have decided to further supplement another state, which is the angular deviation between the localized position and the actual position. This deviation is denoted as $\alpha$, with the following formula:

% \begin{center}
%     $\alpha = \arctan \displaystyle \frac{y_{local} - y_{sim}}{x_{local} - x_{sim}}$
% \end{center}

% With these aforementioned attributes, the model can accurately determine the position localized by vehicle system and use them as a basis for selecting the next action. The results indicate that utilizing these attributes yields promising outcomes, generating various violations and potential violations

% \vspace{0.25cm}
% \noindent\textbf{Perception-related states}
% \vspace{0.25cm}

% Similarly to Localization, Perception is also a vital module with the ability to collect and recognize features of objects around the vehicle. Therefore, the impact of this module on the potential for violations is undeniable. To assess the performance of Perception, we will utilize information obtained from simulations and calculate deviations from the perceived results. Consequently, we observe that these discrepancies occur in various aspects, including:

% \begin{itemize}
%     \item Deviation in position (dis): Even when objects are detected, errors in position can lead to confusion in predictions and decisions regarding the trajectory of the automated vehicle, resulting in violation scenarios. Therefore, this attribute can be used to evaluate the system's state. The formula is as follows, where $x_{per}^i, y_{per}^i$ are perceived coordinates, and $x_{real}^i, y_{real}^i$ are real coordinates.
% \vspace{0.5cm}
%         \begin{center}
%             $dis = \Sigma_{i=0}^{N} \displaystyle \frac{\sqrt{(x_{per}^i - x_{real}^i)^2 + (y_{per}^i - y_{real}^i)^2}}{N}$
%         \end{center}
% \vspace{0.5cm}
%     \item Difference in moving direction (heading): The difference in direction of movement can also be used to indicate the system's state. Misidentifying the direction of movement can cause some type of violations, as improper lane change or improper passing. The formula is as follows, where $he_{per}^i$ is perceived moving directions, and $he_{real}^i$ is real one.
% \vspace{0.5cm}
%         \begin{center}
%             $heading = \Sigma_{i=0}^{N} \displaystyle \frac{|he_{per}^i - he_{real}^i|}{N}$
%         \end{center}
% \vspace{0.5cm}
%     \item Difference in size (size): The impact of size information is somewhat similar to that of position information, as they both determine the potential violation range of obstacles. The formula is as follows, where $h_{per}^i, w_{per}^i, l_{per}^i$ are perceived sizes, and $h_{real}^i, w_{real}^i, l_{real}^i$ are real one.
% \vspace{0.5cm}
%         \begin{center}
%             $size = \sum_{i=0}^{N} \displaystyle \frac{\sqrt{(h_{per}^{i} - h_{gt}^{i})^2 + (w_{per}^{i} - w_{gt}^{i})^2 + (l_{per}^{i} - l_{gt}^{i})^2}}{N}$
%         \end{center}
% \vspace{0.5cm}
    
%     \item Difference in velocity (vel): The speed detected from obstacles will be a crucial factor influencing the autonomous vehicle's subsequent predictions. Therefore, errors in speed could be useful in indicating the system's state. The formula is as follows, where $vx_{per}^i, vy_{per}^i, vz_{per}^i$ are perceived velocity, and $vx_{real}^i, vy_{real}^i, vz_{real}^i$ are real velocity.
% \vspace{0.5cm}
%         \begin{center}
%             $vel = \sum_{i=0}^{N} \displaystyle \frac{\sqrt{(vx_{per}^i - vx_{gt}^i)^2 + (vy_{per}^i - vy_{gt}^i)^2 + (vz_{per}^i - vz_{gt}^i)^2}}{N}$
%         \end{center}
% \vspace{0.5cm}
% \end{itemize}

% Furthermore, for cases where obstacles are not detected, the team adds a large constant value to each attribute. This helps distinguish them from common errors because at this point, the system is unable to accurately detect obstacles.

% \vspace{0.25cm}
% \noindent\textbf{Prediction-related states}
% \vspace{0.25cm}

% Prediction is a module responsible for predicting the trajectory of moving objects in the near future. Depending on the classification, priority, motion scenarios and other external information, each object will be evaluated by a different evaluator. For example, for pedestrians on the road, the Pedestrian Interaction Evaluator will be used to determine their trajectory. That's why we came up with the idea of utilizing the information from this module to generalize AV's operating environment. 

% After reviewing the operation process of this module, we found that exploiting information related to the frequency of use of each evaluator is indeed beneficial, as it provides data regarding the movement scenarios of surrounding objects. Thus, it can provide an overview of the module's activity at the current time. To be clearer, if there are 2 Junction MLP Evaluators and 3 Semantic LSTM Evaluators, Agent can know that scenario has 2 obstacles are moving in junction and 3 obstachles (pedestrians or vehicles) are in caution level. Specifically, we use 12 states corresponding to the frequency of 12 types of evaluators, and 1 state for the Unknown case.

% \vspace{0.25cm}
% \noindent\textbf{Planning\&Control-related states}
% \vspace{0.25cm}

% Planning \& Control are two critical modules directly affecting the vehicle's control process. Planning receives perceived obstalces and predicted trajectories from Perception and Prediction and plans a suitable route for the autonomous vehicle (AV). That's to say, this route has to lead AV to reach the destination and assure driver's safety simultaneously. After planning process, this module transfers control message and makes AV operating.

% To assess the performance of these modules, we employ information obtained from the Control - the results of the Planning process. By this way, the agent will understand how the vehicle is preparing to move and make appropriate action choices. We don't use Planning message because they contain a sequence of waypoints to determine the moving trajectory, and it's hard to extract the new features. So we only utilize the Control module's information. These attributes include:

% \begin{itemize}
%     \item Throttle: A parameter in vehicles that controls the amount of air and fuel entering the engine, thus regulating the engine's power and speed.
%     \item Brake: A specification in vehicles that controls the slowing down or stopping of the vehicle.
%     \item Steering rate: A state measure how quickly the steering wheel is turned, affecting the vehicle's direction and maneuverability.
%     \item Steering target: A factor in vehicles that indicates the desired direction or angle to which the steering system should aim, guiding the vehicle's path.
%     \item Acceleration: A criterion provides the rate at which the vehicles's speed increases or decreases.
%     \item Gear: A metric that decribes vehicle's driving mode.
% \end{itemize}

\subsection{Behavior-based Action Space}
The actions used in the system will be operations that change the state of the testing environment, such as switching states regarding time or weather conditions. In DeepCollision , their action space includes actions related to behaviors, colors, and classifications of vehicles. However, during experimentation, we did not observe the impact of factors such as the shape and color of the vehicle on the probability of generating violations. The results yielded various types of vehicles and colors being chosen but did not bring about effectiveness and reduced scenario diversity. Therefore, to narrow down the learning scope and improve efficiency, we focus on the behaviors of the dynamic objects (pedestrian or other vehicles) to generate diverse and scenariors. Such behaviors include:

\begin{itemize}
    \item Overtaking: Vehicles passing the automated one.
    \item Drive ahead: Vehicles moving in front of the automated one.
    \item Cross-road: Vehicles cutting across the roadway.
    \item Drive opposite: Vehicles moving in the opposite direction to the automated vehicle.
\end{itemize}

Additionally, for pedestrians, we will use actions allowing them to cross the road from left to right and vice versa. Objects will be added to the environment at two different distances: near and far, to ensure realism without being too close as in DeepCollision.

We have observed that time and weather have certain impacts on the scenario's danger level. However, these impacts are not significant and do not require excessive focus. Therefore, we will limit their occurrence frequency on the system in two ways:

\begin{itemize}
    \item In the last 5 steps, no two actions related to time or weather are performed.
    \item If the action is similar to the last time/weather related action performed, they will be reselected.
\end{itemize}

\subsection{Violation, Collision and Diversity Reward:}
After observing the environment states $S_t$ and implementing action $A_t$, agent changes to next states $S_{t+1}$ and reveices reward for current action. The reward is responsible for guiding agent to choose appropriate action to optimize objectives. In MoViTe, the reward indicates how challenging the recent action was, and if it caused a violation or collision, it also shows the diversity of that scenario. To be clearer, we implement reward in Multi-objectives form, with three components being violation probability, collisison probability and diversity level.

\subsubsection{Violation Probability}
Violation Probability Reward is one of two main objectives optimized by MoViTe. This reward demonstrates the potential the current action brings in creating challenging driving scenario. That's to say, if violation probability reward less or equal to zero, it has no chance in creating new infraction. If this reward equals to 1, it certainly causes extremely violation. In the remain cases, current scenario is likely to result in breaking traffic rules.

In section \ref{violation-modeling}, we define 3 types of behaviors, 7 types of violations, and the formulas used to evaluate their likelihood. Then, we calculate violation probability reward based on each violation rate. After each action, AV runs in 6 seconds and collects data to figure out evaluating metrics. This time period will be divided into 12 parts, each part lasts 0.5 seconds and we measures violation rate of each violation after it. Probability of violation i in part j denoted by $\displaystyle VioRate_{i}^{j}$, and the result we obtained after the evaluation period is $\displaystyle \left \{ VioRate_{i}^{j} | 0 \leq i \leq N_{vio}, 0 \leq j \leq 11  \right \}$. Then, \tool chooses the maximum rate of each violation throughout the evaluation period to assess the action. Let's set final violation rate $VioRate^{final}$, we have the formula:

\begin{center}
    $\displaystyle VioRate_{i}^{\text{final}} = \max_{j=0}^{12} \left( VioRate_{i}^{j} \right), \quad \text{for } 0 \leq i \leq N_{vio}$
\end{center}

After obtaining this final value, \tool conducts an overall assessment of the probability of occurrence of violations. It means that we aggregates each violation and return an overall value, or violation probabilty reward. If a type of violation does not occur, \tool receives a reward equivalent to the probability of that violation occurring. However, if the violation does happen, we will add one more reward point to encourage the system to continue in that direction. The formula is as follows:

\begin{center}
    \(VioReward_i =
    \begin{cases} 
        VioRate_i^{final} \text{ , if } VioRate_i^{final} < 1.0 \\
        VioRate_i^{final} \text{ + } 1 \text{ ,} \text{ else}
    \end{cases}\)
\end{center}


After that, we calculate the average value of the rewards to evaluate \tool's ability to generate violation scenarios:

\begin{center}
    $\displaystyle VioProbReward = max(VioReward) + \frac{2 - max}{2 \cdot (N_{vio}^{+} - 1)} \left(\sum_{i}^{N_{vio}} VioReward_i \cdot w_i - max \right)$
\end{center}

where $N_{vio}^{+}$ is the number of violation whose occuring probability greater than zero; and $w_i$ is weight of violation i, judges it's contribution in final value. However, in cases where \tool performs poorly by choosing actions that do not result in significant violation rates, we will assign a penalty value of -1. Therefore, the general formula for VioProbReward is as follows:

\begin{center}
    \(\displaystyle VioProbReward = 
    \begin{cases}
        -1 \text{ , if } VioProbReward < 0.2 \\
        VioProbReward \text{ , else}
    \end{cases}
    \)
\end{center}

In a general case, we usually consider violation weights equally and set these weights to $\frac{1}{N_{vio}}$. However, it may lead to bias towards some certain types of violations because it's easy for them to occur or the underlying scenarios could favor them. As a result, they reduce the diversity of violations generated. 

To balance these frequencies, we apply a continuous weight adjustment method. The main idea is that when a violation occurs, we decrease its weight by a certain amount and evenly increase other violations's weight. By this way, the violation occurs more frequently has lower weight, or has a smaller impact on violation probability reward while the others has higher one. Thus, \tool should learn and try to generate more challenging violation. 

Initially, all the weight value is set to 1/7. After implementing each action, \tool calculate violation rate of each violation. If a violation occurs, we decrease its weight by $w_{decay} \%$. In cases where many violation happen simultaneously, the reduction amount will be accumulated. Then, this amount is divided equally to other violation weights. Specifically, those weights will rise about $added\_weight$, whose formula is as follow:

\begin{center}
    $added\_weight = \displaystyle \frac{total\_decay}{rest}$
\end{center}
where $total\_decay$ is reduced amount and rest is number of non-occured violation. In \tool, we set added $w_{decay}$ = 10 which means that if one violation occurs, its weight will be decreased by 10 percent. 

Violation Probability is an important objective that lead \tool to more challenging scenarios. With formulas mentioned above, we could calculate overall violation probability based on each individual  violation rate. Moreover, to equalize occurence frequencies, we continuous adjust violation's weight such that scenarios happen more regularly would be reduced more while those occuring less are increased. Thanks to this method, we could ensure diversity among many types of violation. Besides, utilizing a weighting mechanism, \tool can be adjusted to focus on specific types of violations that are beneficial to the problem.  

\subsubsection{Collision Probability}
After evaluating the sub-goal of the ability to generate violations, we will need to calculate the reward for the main objective, specifically the collision probability of the scenario. When \tool selects an action and executes it in the test environment, a higher value indicates that \tool is performing well in creating severe collisions. Similar to many other studies, the collision probability will be calculated based on the values of Safety Distance and Current Distance. We will project these values onto the two axes of the UTM coordinate system to obtain EaSD, NoSD, EaCD, and NoCD along the two axes. The formula for collision probability is then as follows:

\begin{center}
    \(EaProC = \displaystyle \frac{EaSD - EaCD}{EaSD}\) \\[0.25cm]
    \(NoProC = \displaystyle \frac{NoSD - NoCD}{NoSD}\) \\[0.25cm]
    \(ProC = EaProC \cdot NoProC\)
    
\end{center}

The higher the collision probability at this moment, the greater the amount of reward that \tool will receive. Specifically, if \tool creates a collision, it means the agent has chosen a highly effective action. Therefore, we will give a reward to the agent to encourage further development in this direction. Therefore, the collisison probability reward value will be represented by the following formula:

\begin{center}
    \(ProCReward = 
    \begin{cases}
        ProC \text{ , if } ProC < 1.0 \\
        ProC + 1 \text{ , else}
    \end{cases}
    \)
\end{center}

\subsubsection{Diversity Level}

In addition to generating challenging violation, \tool also directs to optimize scenario diversity. This diversity aspect attracts a lot of attention from researchers and developers. Indeed, many recent studies just have focused on generating violation scenarios without paying attention to their diversity. The result is that there are too many violations generated, but the diversity is not very high.

In recent years, there have had several attempts in eliminating duplicate scenarios, and it happened in post-processing stage. Our approach is quite different from others. We apply diversity evaluating method in calculating reward stage and use metrics as reward for agent, called Diversity Level. 

Main idea is that we divided a scenario into many frames represented by a vector of environment states. After performing calculations on these vectors, we will compare them with generated scenarios to assess their diversity. If the distance from the current scenario to the previous ones is small, it could be a duplicate violation and agent would receive a penalty for this action. On the contrary, it is quite different from the others, indicating an increase in diversity. So a reward point would be given to the agent.

Assuming that \tool has already implemented action $A_i$ in state $S_i$, and now is calculating reward and transitioning to next state $S_{t+1}$. At each time part, we extract many attributes to represent current operating environment. Regarding to external environment, we get traffic light color, weather, time, and obstacles information. To be clearer, obstacles information contains distance to ego, rotation, velocity, acceleration and type (pedestrian or vehicle). We collect data from three nearest obstacles because they have a significant impact on the vehicle's violation probability. Considering the ego, we utilize heading, velocity, acceleration and brake. Finally, we get violation type as a state if a violation occurs and set it to 0 in the opposite case.

After evaluating time, we obtained a scenario composed of 12 frames represented for recent scenario. If a violation did not occur, we set this reward to a value that does not affect the result (i.e 0). In the opposite case, \tool uses sliding window w to group consecutive vectors into segments. We do this to break down the scenario into smaller components, making it easier to compare. If the first factor of one group is $x_i$, this segment is denoted by $\{ x_i, x_{i+1}, ..., x_{x+w-1} \}$. Then, we acquired $\displaystyle \frac{12}{w}$ segments in a scenario. After that, \tool takes place a lot of statistical measures to merge vectors in one segment. They could be mean, minimum, maximum, mean\_change, mean\_abs\_change, v.v. Let's set M is the number of states, and D is the number of statistical features. The result we got after merging phase is vector $seg_i$ with the size D x M. Then, current scenario represented as follow:

\begin{center}
    $\displaystyle Scenario = \{seg_i | 0 \leq i \leq \frac{12}{w}\}$
\end{center}

However, the range of attribute values still varies significantly, for example, between position and weather, and they influence the comparison process. To address this problem, we implement Clustering Algorithm (i.e Kmean, DBSCAN) to distribute segments to clusters. By this way, similar segments could be divided into the same group and we use cluster id to represent for these segments. Then, a scenario is denoted by clusters's id as follow: 

\begin{center}
    $Scenario = \{ seg\_cls_i | 0 \leq i \leq \frac{12}{w} \}$
\end{center}

where $seg\_cls_i$ is cluster's id of segment i. At this point, we have a scenario represented by states with values that are not significantly different from each other. Finally, we adopt distance-based formulas to assess scenario diversity (Hamming distance used in this paper). Then, Diversity Level is defined as follow:

\begin{center}
    $div\_level = \displaystyle \frac{1}{N_{sce}} \sum_{i=0}^{N_{sce}} dis(Scenario_{curr}, Scenario_i)$
\end{center}
where $N_{sce}$ is the number of generated scenarios, $Scenario_{curr}$ is current scenario's vector. If $div\_level$ got a high value, it means that we obtained a new violation, and then update to generated set. But on contrary case, this distance is really low, and it is a penalty for failed the task.

After measures both Violation Probability Reward, Collision Probability Reward and Diversity Reward, we combine them to acquire value for agent. The final reward is denoted as follow:

\begin{center}
    $reward = vio_w \cdot VioProbReward + col_w \cdot ProCReward + div_w \cdot div\_level$
\end{center}
where $vio_w$, $col_w$ and $div_w$ is weight for violation probability reward, collision probability reward and diversity reward, respectively. Depending on project requirements, we can adjust these weights to prioritize objectives.



==> 3.formulation/actions_backup.tex <==
\subsection{Actions to Configure the Environments}
\label{sec:action}

The operational environment of an AV is highly complex and influenced by various factors, including time, weather, obstacles, etc. Each time these factors change, they can potentially lead to severe collisions in reality. In this context, the actions performed by agents aim to modify the components of the environment in a way that makes collisions more likely. The components affected by \tool are listed in Table\ref{tab:configurable} . However, during experimentation, we did not observe the impact of factors such as type, size and color of the vehicle on the probability of generating collisions. The results yielded various types of vehicles and colors being chosen but did not bring about effectiveness and widened search space excessively. Therefore, to narrow down the learning scope and improve efficiency, we just focus on the behaviors of the dynamic objects (pedestrian or other vehicles) to generate challenging scenarios. Such behaviors include:

\begin{itemize}
    \item Overtaking: Vehicles passing the automated one.
    \item Drive-ahead: Vehicles moving in front of the automated one.
    \item Cross-road: Vehicles cutting across the roadway.
    \item Drive opposite: Vehicles moving in the opposite direction to the automated vehicle.
\end{itemize}

For all behaviors, the type and color of the vehicle will be randomly selected from the options listed in Table \ref{tab:configurable}. Regarding each behavior, we focus on the following key factors: distance, speed, moving direction and lane change decisions. These factors may vary depending on the type of behavior, but they must still ensure that the vehicle is generated at a safe distance from other traffic. The speed of the NPCs is typically set to 20 m/s to approach the AV quickly. Additionally, they can be placed in different positions (left, right, or in the same lane as the ego vehicle) with appropriate lane change decisions (left - change to the right lane, right - change to the left lane, etc). However, there are several constraints as follows:

\begin{itemize}
    \item For overtaking, NPC vehicles will be generated behind the AV, with the distance depending on the type of vehicle. Smaller vehicles (Sedan, SUV, etc.) will be generated 5 meters away, while larger vehicles (Box Truck, School Bus) will be generated 10 meters away from the AV. 

    \item For driving ahead, the distance values are divided into two categories: near and far. For the near distance, NPCs will appear 12 meters in front for smaller vehicles and 15 meters for larger vehicles. For the far distance, the common distance is set to 50 meters. Unlike others behaviors, the goal of this behavior is to just create vehicles moving in front of the ego vehicle and maintain the suitable distance. So the speed for these vehicles are set to 10 m/s.

    \item For drive-opposite, vehicles will be generated in front of the ego vehicle with two distance categories similar to drive-ahead. However, they need to be generated at greater distances. Specifically, for the near case, the distance from the ego vehicle is 20 meters, while for the far case, it is 50 meters. 

    \item For cross-road, vehicles will be generated in front of the ego vehicle and will perform a lane change into the ego’s current lane to create a dangerous situation by crossing. Similar to drive-ahead and drive-opposite, cross-road vehicles will appear at two distances: near and far. For the near case, they are positioned 12 meters and 17 meters away for smaller and larger vehicles, respectively. For the far case, the distances are 25 meters and 30 meters, respectively.
    
\end{itemize}

Additionally, for pedestrians, we will use actions allowing them to cross the road from left to right and vice versa. The position of pedestrians will be 40 meters from the ego vehicle. During experiments, actions involving pedestrians are more likely to cause collisions compared to other options, and thus can impact the agent’s decisions. Therefore, we will design these actions to be less likely to cause collisions while still ensuring their realism.

We have observed that time and weather have certain impacts on the scenario's danger level. However, these impacts are not significant and do not require excessive focus. Therefore, we will limit their occurrence frequency on the system in two ways:

\begin{itemize}
    \item In the last 5 steps, no two actions related to time or weather are performed.
    \item If the action is similar to the last time/weather related action performed, they will be reselected.
\end{itemize}

\begin{table}[!t]
\centering
\caption{Configurable environment parameters}
\label{tab:configurable}
\begin{tabular}{llp{4cm}}\toprule
Type          & Parameter  & Configuration \\ \midrule
\multirow{3}{*}{Weather}    
              & Rain       & None, Light, Moderate, Heavy \\
              & Fog        & None, Light, Moderate, Heavy \\
              & Wetness    & None, Light, Moderate, Heavy \\ \midrule
Time of Day   & timeOfDay  & Morning, Noon, Night \\ \midrule
\multirow{4}{*}{Pedestrian} 
              & Position   & $(x_0^p, y_0^p, z_0^p)$ \\
              & Rotation   & $(x_0^r, y_0^r, z_0^r)$ \\
              & Speed      & $v_0$ \\
              & Behavior   & CrossRoad \\ \midrule
\multirow{6}{*}{NPC Vehicle} 
              & Position   & $(x_0^p, y_0^p, z_0^p)$ \\
              & Rotation   & $(x_0^r, y_0^r, z_0^r)$ \\
              & Speed      & $v_0$ \\
              & Type       & SUV, Sedan, Jeep, Hatchback, Schoolbus, BoxTruck \\
              & Color      & Pink, White, Red, Black, Sky-blue, Yellow\\
              & Behavior   &  DriveAhead, DriveOpposite, CrossRoad, Overtake  \\ \bottomrule
\end{tabular}
\end{table}



==> 5.results/chart_action_analysis.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/action_analysis_fine_grained.png}
        \caption{}
        \label{fig:state_road1}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/action_analysis_behavior_based.png}
        \caption{}
        \label{fig:state_road3}
    \end{subfigure}%
    % \includegraphics[width=\linewidth]{images/state_analysis.png}
    \caption{Action Analysis Results. a) Fine-grained Action-space evaluation b) Behavior-based Action-space evaluation. They evaluated based on the chosen proportion of action group in experiments}
    \label{fig:action_analysis_charts}
\end{figure}

==> 5.results/chart_intrinsisc_analysis.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/intrinsic_analysis_action.png}
    \caption{PER Evaluation. The blue line represents the selection frequency of DDQN, while the red line represents that of DDQN + PER.}
    \label{fig:per_evaluation}
\end{figure}

==> 5.results/model_analysis.tex <==
\subsubsection{Model Analysis}

\input{5.results/tab_intrinsic_analysis}

We evaluated the contributions of \tool's RL model to its overall performance. 
% Specifically, we assess two components: DDQN and PER. 
In this experiment, we compare the performance of \tool using DQN as a baseline, and \tool using DDQN with and without PER. The performance is measured in term of \textit{\#Collision} and \textit{\%Action}. While \textit{\#Collision} specifies the effectiveness of the approach, \textit{\%Action} refers to the portion of actions are selected, which denotes the ability of attempting a diverse actions of the models.
The results are presented in Table \ref{tab:intrinsic_analysis_model}. 


Notably, \tool with DDQN outperformed DQN by generating over 55\% more collisions. This highlights the improvements achieved by using DDQN in a complex and dynamic environment like ADS testing, which involves a lot of noisy data and inaccurate estimations. However, the \textit{\%Actions} for both models is only 80\% indicating that they have not yet achieved optimal effectiveness. After incorporating PER, \tool's performance significantly improved. Specifically, the \textit{\%Actions} of DDQN+PER reached 95.5\%, a 19.3\% improvement compared to when PER was not used. Additionally, after integerating PER, the number of collisions obtained remain consistent, only a 4\% of difference. This difference is relatively small and could be attributed to various factors, such as the randomness of the $\epsilon$-Greedy Policy or the characteristics of the map. 
The consistency in obtained collisions and the increased action selection rate indicate that incorporating PER significantly enhanced the model's learning capability while maintaining stability in generating critical scenarios. 


By analyzing the actions selected by different variants of \tool, we found that a significant bias in DDQN towards certain actions. For instance, with DDQN, the most frequent action was chosen 33.4\% of the time,
while the second and third most frequent actions were selected at rates of 7.9\% and 5.2\%, respectively.
Meanwhile, integrating PER allowed \tool to explore a more diverse set of actions and reduce this bias toward specific choices. In particular, with PER, the selection rates for three most frequent actions were more balanced, at approximately 9.3\% each.



% To observe the impact of PER on \tool, we evaluated the frequency of the top-3 selected actions for each configuration. The results are shown in Fig~\ref{fig:per_evaluation}. The blue line represents the selection rate of DDQN, while the red line represents DDQN+PER. From this, we can see a significant gap between \%1stAction and \%2ndAction by DDQN, approximately 22.45\%. This reflects a bias in DDQN towards a certain action during the experiment. The random selection of actions from the Buffer Memory caused the model to repeatedly learn one particular action, leading to an excessive focus on this action and a loss of scenario diversity. In contrast, with PER, \tool proved to be highly effective, as the gap between \%1stAction, \%2ndAction, and \%3rdAction was only 1-3\%. Thus, \tool showed no bias toward any particular action, allowing it to evaluate different actions fairly, which enhanced the diversity of collision scenarios. This is also reflected in the \tool's action selection rate reached 95.5\%.

% Finally, based on the above evaluations, the two components, DDQN and PER, improved the model's learning ability by producing high \#Collisions and significantly broadening the learning scope. The actions were better utilized and yielded stable results without being distracted by other trivial actions.

% \input{5.results/chart_intrinsisc_analysis}





==> 5.results/realistic.tex <==
\subsubsection{Realism of the Generated Scenarios}

==> 5.results/tab_eps_analysis.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Impact of $\epsilon$ threshold on \tool's performance}\label{tab:eps_analysis}
\scriptsize
\begin{tabular}{l|rrr}\toprule
$\theta_\epsilon$ & \#Collisions &TTC \\\midrule
0.0 &14.4 &31.3  \\
0.1 &12.4 &40.3  \\
0.2 &16.2 &35.3  \\
0.5 &10.0 &35.6  \\
0.8 &7.6 &39.9  \\
\bottomrule
\end{tabular}
\end{table}

==> 5.results/tab_intrinsic_analysis.tex <==
\begin{table}\centering
\caption{Performance of generating critical scenarios using difference model architectures}
\label{tab:intrinsic_analysis_model}
\scriptsize
\begin{tabular}{l|rrr}\toprule
\textbf{Models} &\textbf{\%Action (\%)} &\textbf{\#Collisions}\\\midrule
DQN &80.0 &12.6 \\
DDQN &80.0 &19.6 \\
DDQN + PER &\textbf{95.5} &\textbf{18.9} \\

\bottomrule
\end{tabular}
\end{table}

==> 5.results/tab_otp.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Impact of $OTP$ values on \tool's performance}\label{tab:otp_analysis}
\scriptsize
\begin{tabular}{c|rrr}\toprule
\textbf{OTP (s)} &\textbf{\#Collisions} &\textbf{TTC}  \\\midrule
4 &1.2 &40.70  \\
6 &11.8 &25.85  \\
8 &7.2 &28.89  \\
\bottomrule
\end{tabular}
\end{table}

==> 5.results/tab_rcol.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Impact of $R_{col}$ values on \tool's performance}\label{tab:rcol_analysis}
\scriptsize
\begin{tabular}{r|rrrr}\toprule
\textbf{$R_{col}$} &\textbf{\#Collisions} &\textbf{TTC} \\\midrule
1.0 &2.7 &26.06  \\
2.5 &12.0 &48.33  \\
7.5 &13.4 &32.60  \\
10.0 &11.6 &19.91\\
\bottomrule
\end{tabular}
\end{table}

==> 8.variable.tex <==
% \section{Variables}

% \subsection{Car status variable}

\input{table/car_status}

% \subsection{Driving status variable}

\input{table/driving_status}

% \subsection{Environment status variables}

\input{table/environment_status}

% \subsection{Road status variables}

\input{table/road_status}

% \subsection{Traffic status variables}
\input{table/traffic_status}

% \subsection{Traffic signal status variables}

\input{table/traffic_signal_status}

% \subsection{Utility Function}

\input{table/utility_function}

==> 9.formula.tex <==
\section{Safe Driving Violation Formulation}

\subsection{Passing Violation (Acceleration)}

\noindent\underline{\textbf{Passing in any section}}

\subsubsection{Unsafe passing on left (ORS 811.410)}
\begin{center}
    $EGO.isPassing \wedge onLft(EGO, NPCAhd) \wedge ((disTo(EGO, NPCAhd) < SD) \vee \lnot hasClrView \vee \lnot freeOfTrf)$
\end{center}

\subsubsection{Unsafe passing on right (ORS 811.415)} 
\begin{center}
    $EGO.isPassing \wedge onRgt(EGO, NPCAhd) \wedge (\lnot (NPCAhd.turnSig \vee onLft(NPCAhd, centLine)) \vee  (rmnWdAhd < 2 \cdot EGO.width) \vee onRgt(EGO, rightCurb) \vee (disTo(EGO, NPCAhd) < SD))$
\end{center}

\noindent\underline{\textbf{Passing in special zone}}

\subsubsection{Failure to yield right of way within roundabout (ORS 811.292)}
\begin{center}
    $ on(EGO, rndabt) \wedge (EGO.isPassing \vee ((NPCAhd.turnDecision \neq None) \wedge  \lnot yldDec(NPCAhd)) $
\end{center}

\subsubsection{Passing in no passing zone (ORS 811.420)}
\begin{center}
    $EGO.isPassing \wedge on(EGO, npZone) \wedge (EGO.turnDec \neq  left) \wedge \lnot hasObsAhd$
\end{center}

\subsubsection{Passing stopped vehicle at crosswalk (ORS 811.020)}
\begin{center}
    $EGO.isPassing \wedge (NPCAhd.spd = 0) \wedge hasCrwkAhd$
\end{center}

\subsubsection{Unsafe passing of person operating bicycle (ORS 811.065)}
\begin{center}
    $ EGO.isPassing \wedge onLft(EGO, NPCAhd) \wedge ((disTo(EGO, NPCAhd) < SD) \vee \lnot how hasObsAhd) $
\end{center}


\subsection{Direction Changing Violations (Direction Changing)}

\underline{\textbf{Lane Changing Violation}}

\subsubsection{Unlawful or unsignaled change of lane (ORS 811.375)}
\begin{center}
    $EGO.isLaneChanging \wedge ((disTo(EGO, NPC) < SD) \vee \lnot EGO.turnSig \vee (EGO.sigDur < 30))$
\end{center}

\subsubsection{Failure of merging driver to yield right of way (ORS 811.285)}
\begin{center}
    $ EGO.isLaneChanging \wedge on(NPCBack, EGO.predLane) \wedge \lnot yldDec(NPCBack) $
\end{center}

\noindent\underline{\textbf{Left Turning Violation}}

\subsubsection{Dangerous left turn (ORS 811.350)}
\begin{center}
    $ EGO.isTurning \wedge (EGO.turnDec = left) \wedge (disTo(EGO, NPCOppo) < SD) \wedge \lnot yldDec(NPCOppo) $
\end{center}

\subsubsection{Failure to use special left turn lane (ORS 811.345)}
\begin{center}
    $ EGO.isTurning \wedge (EGO.turnDec = left) \wedge \lnot (specLftLane = NULL) \wedge \lnot on(EGO, specLftLane) $
\end{center}


\subsubsection{Illegal U-Turn (ORS 811.365) }
\begin{center}
    $ EGO.isTurning \wedge (EGO.turnDec = left) \wedge (EGO.predLane \parallel curLane) \wedge (EGO.predLane.dir \cdot curLane.dir < 0) \wedge \lnot hasClrView(EGO.predLane)$
\end{center}

\subsubsection{Improperly executed left turn (ORS 811.340)}
\begin{center}
    $ EGO.isTurning \wedge (EGO.turnDec = left) \wedge (\lnot on(EGO, extmLftLane) \vee \lnot onLft(EGO, inter))$
\end{center}

\subsubsection{Failure to yield right of way at uncontrolled T intersection (ORS 811.277)}
\begin{center}
    $ EGO.isturning \wedge on(EGO, t\_inter) \wedge (EGO.moveDir \cdot NPCAhd.moveDir = 0) \wedge (EGO.turnDecision = right) \wedge (EGO.predLane = NPCAhd.curLane) \wedge \lnot yldDec(NPCAhd) $
\end{center}

\noindent \underline{\textbf{Right Turning Violation}}

\subsubsection{Improperly executed right turn (ORS 811.355)}
\begin{center}
    $ EGO.isTurning \wedge (EGO.turnDec = right) \wedge (disTo(EGO, rightCurb) > \theta_3)$
\end{center}

\noindent\underline{\textbf{Turning Violation}}

\subsubsection{Unlawful or unsignaled turn (ORS 811.335)}
\begin{center}
    $ EGO.isTurning \wedge (EGO.turnDec \neq None) \wedge ((disTo(EGO, NPC) < SD) \vee \lnot EGO.turnSig \vee EGO.sigDur < 30)$
\end{center}

\noindent\underline{\textbf{Backing Violations}}


\subsubsection{Illegal backing (ORS 811.480)}
\begin{center}
    $EGO.isBacking \wedge ((disTo(EGO, NPCBack) < SD) \vee (\sum\Delta NPCBack.pos < \theta_1))$
\end{center}

\subsection{Cruising Violations (Acceleration, !Direction Changing)}

\noindent\underline{\textbf{Cruising in special zone/lane}}

\subsubsection{Crossing center line on two-way, four-lane road (ORS 811.310)}
\begin{center}
    $EGO.isCruising \wedge (rdTyp = two\_way) \wedge (numLane \geq 4) \wedge onLft(EGO, centLine) \wedge \lnot (hasObsAhd \wedge (freeOfTrf \vee EGO.turnDec = left))$
\end{center}

\subsubsection{Driving on highway divider (Driving on highway divider)}
\begin{center}
    $EGO.isCruising \wedge (extmLftLane.boundary.type = double\_solid\_yellow) \wedge (rdTyp = highway) \wedge isInter(EGO, extmLftLane.boundary)$
\end{center}

\subsubsection{Driving on left on curve or grade or at intersection or rail crossing (ORS 811.305)}

\begin{center}
    $EGO.isCruising \wedge rdTyp \in  \{ curve, grade, inter, rail crossing \} \wedge onLft(EGO, centLine)$
\end{center}

\subsubsection{Driving through safety zone (ORS 811.030)}

\begin{center}
    $EGO.isCruising \wedge on(EGO, sftyZone)$
\end{center}

% \subsubsection{Failure to drive on right}

% \begin{center}
%     $ EGO.isCruising \wedge (rmnWdAhd > 2 \cdot EGO.width) \wedge onLft(EGO, centLine) $
% \end{center}

\subsubsection{Failure to drive to right on divided highway (ORS 811.320) }

\begin{center}
    $EGO.isCruising \wedge (extmLftLane.boundary.type = double\_solid\_yellow) \wedge (rdTyp = highway) \wedge onLft(EGO, extmLftLane.boundary)$
\end{center}

\subsubsection{Failure to obey one-way designation (ORS 811.270)}

\begin{center}
    $EGO.isCruising \wedge EGO.moveDir \cdot curLane.dir < 0$
\end{center}

\subsubsection{Operation of motor vehicle on bicycle trail (ORS 811.435)}

\begin{center}
    $ EGO.isCruising \wedge on(EGO, bicTrail)) $
\end{center}

\subsubsection{Unlawfully operating low-speed vehicle on highway (ORS 811.512 )}

\begin{center}
    $EGO.isCruising \wedge (rdTyp = highway) \wedge (EGO.spdLim <= 40)$
\end{center}

\noindent\underline{\textbf{Cruising in normal zone/lane}}

\vspace{0.25cm}

\noindent\textbf{Normal speed}

\vspace{0.25cm}

\noindent \textit{In one lane}

\subsubsection{Following too closely (ORS 811.485)}

\begin{center}
    $ EGO.isCruising \wedge on(NPCAhd, curLane) \wedge disTo(EGO, NPCAhd) < 5 $
\end{center}

\subsubsection{Failure to drive on right of approaching vehicle (ORS 811.300)}

\begin{center}
    $EGO.isCruising \wedge (rdTyp = two\_way) \wedge (numLane <= 2) \wedge aprc(NPCAhd, EGO) \wedge onLft(EGO, NPCAhd) $
\end{center}

\subsubsection{Obstructing cross traffic (ORS 811.290) (?)}

% \begin{center}
    
% \end{center}

\subsubsection{Failure of driver entering roadway to yield right of way (ORS 811.280)}
\begin{center}
    $ EGO.isCruising \wedge (EGO.moveDir \nparallel EGO.predLane.dir) \wedge \lnot yldDec(NPCAhd) $
\end{center}

\noindent \textit{In many different lanes}

\subsubsection{Depriving motorcycle or moped of full lane (ORS 811.385)}
\begin{center}
    $EGO.isCruising \wedge on(EGO, motorLane) \wedge on(EGO, adjLane(motorLane)) \wedge disTo(EGO, NPCBack) < SD$
\end{center}

\subsubsection{Failure to drive within lane (ORS 811.370)}

\begin{center}
    $ EGO.isCruising \wedge on(EGO, adjLane(curLane)) \vee (EGO.isLaneChanging \wedge (disTo(EGO, NPC) < SD)) $
\end{center}

\noindent\textbf{Low speed}

\subsubsection{Failure of slow driver to drive on right (ORS 811.315) }

\begin{center}
    $ EGO.isCruising \wedge EGO.spd < avg(NPC.spd) \wedge \lnot on(EGO, extmRgtLane) $
\end{center}

\subsubsection{Failure of slower driver to yield to overtaking vehicle (ORS 811.425) (?)}

% \begin{center}
    
% \end{center}

\subsection{Overlap Violations (Acceleration, Direction Changing)}

\noindent\underline{\textbf{Traffic Signal Violation}}

\subsubsection{Driver failure to obey traffic control device (ORS 811.265)}

\noindent\textbf{Green Signal Violation}
\vspace{0.25cm}

\noindent Green signal:
% \vspace{0.25cm}

\begin{center}
    $(trfLig.color = green) \wedge (trfLig.type = circular) \wedge on(NPCAhd, inter) \wedge \lnot yldDec(EGO, NPCAhd)s$
\end{center}

\noindent Green arrow signal:
% \vspace{0.25cm}

\begin{center}
    $\forall trfLig, (trfLig.color = green) \wedge (trfLig.type = arrow) \wedge (EGO.moveDir \neq trfLig.dir)$
\end{center}

\noindent\textbf{Yellow Signal Violation}
\vspace{0.25cm}

\noindent Steady circular yellow signal
\begin{center}
    $(trfLig.color = yellow) \wedge (trfLig.type = circular) \wedge (\lnot EGO.isStopping \wedge disTo(EGO, NPCAhd) < SD)$
\end{center}

\noindent Steady yellow arrow signal (?)
\begin{center}
    $(trfLig.color = yellow) \wedge (trfLig.type = arrow) \wedge (\lnot EGO.isStopping \wedge ((EGO.moveDir \neq trfLig.dir) \vee (disTo(EGO, NPCAhd) < SD)$
\end{center}

\noindent Flashing circular yellow signal
\begin{center}
    $(trfLig.color = yellow) \wedge (trfLig.type = flashing\_ircular) \wedge disTo(EGO, NPCAhd) < SD$
\end{center}

\noindent Flashing yellow arrow signal (?)

\noindent\textbf{Red Signal Violation}
\vspace{0.25cm}

\noindent Steady circular red signal
\begin{center}
    $(trfLig.color = red) \wedge (trfLig.type = circular) \wedge \lnot EGO.isStopping$
\end{center}

\noindent Steady red arrow signal
\begin{center}
    $(trfLig.color = red) \wedge (trfLig.type = arrow) \wedge (trfLig.dir = EGO.moveDir) \wedge \lnot EGO.isStopping$
\end{center}

\noindent Flashing circular red signal
\begin{center}
    $(trfLig.color = red) \wedge (trfLig.type = flashing\_circular) \wedge (\lnot EGO.isStopping \vee (EGO.isStopping \wedge !hasClrView)$
\end{center}

\noindent\textbf{Stop Signs}
\vspace{0.25cm}

\noindent Stop Signs
\begin{center}
    $stopSign \wedge (\lnot EGO.isStopping \vee (on(NPCAhd, inter) \wedge \lnot yldDec(NPCAhd)))$
\end{center}

\begin{center}
    
\end{center}

\noindent\underline{\textbf{Vehicle Signal Violation}}

\subsubsection{Failure to use appropriate signal for turn, lane change, stop or exit from roundabout (ORS 811.400)}
\begin{center}
    $ on(EGO, rndabt) \wedge (((turnDec \neq None) \wedge (turnSingal \neq turnDec)) \vee ((isStopping \vee isDeceleration) \wedge \lnot brkSig)) $
\end{center}

\subsubsection{Failure to signal with lights (ORS 811.405)}
\begin{center}
    $ \lnot hasClrView \wedge (((turnDec \neq None) \wedge (turnSingal \neq turnDec)) \vee ((isStopping \vee isDeceleration) \wedge \lnot brkSig)) $
\end{center}

\noindent\underline{\textbf{Driving in special zone}}

% \noindent\textbf{Intersection}

\subsubsection{Failure to yield right of way at uncontrolled intersection (ORS 811.275)}
\begin{center}
    $ on(EGO, inter) \wedge \lnot trfLig \wedge onRgt(EGO, NPCAhd) \wedge \lnot yldDec(NPCAhd) $
\end{center}

% \noindent\textbf{Sidewalk}
\subsubsection{Failure to stop when emerging from alley, driveway or building (ORS 811.505)}

\begin{center}
    $ \lnot EGO.isDeceleration \wedge (curLane \nparallel EGO.predLane) \wedge (swkAhd \vee \lnot hasClrView) $
\end{center}

\subsubsection{Failure to yield to bicyclist on sidewalk (ORS 811.055)}
\begin{center}
    $ on(EGO, swkAhd) \wedge \lnot yldDec(bicAhd) $
\end{center}

\subsubsection{Failure to yield to pedestrian on sidewalk (ORS 811.025)}
\begin{center}
    $ on(EGO, swkAhd) \wedge \lnot yldDec(pedesAhd) $
\end{center}

% \noindent\textbf{Traffic island}
\subsubsection{Driving wrong way around traffic island (ORS 811.330)}

\begin{center}
    $EGO.isCruising \wedge onLft(EGO, rotTrfIsl)$
\end{center}

% \noindent\textbf{Three-lane road}
\subsubsection{Improper use of center lane on three-lane road (ORS 811.380)}
\begin{center}
    $ (numLane = 3) \wedge adjLane \in \{extmLftLane, extmRgtLane\} \wedge (curLane.dir \cdot EGO.moveDir < 0) \wedge \lnot EGO.isPassing \wedge \lnot (EGO.turnDec = left)  $
\end{center}

% \noindent\textbf{Bicycle trail}
\subsubsection{Failure to yield to rider on bicycle lane (ORS 811.050)}
\begin{center}
    $ on(EGO, bicTrail) \wedge \lnot yldDec(bicAhd) $
\end{center}

\noindent\underline{\textbf{Driving in normal lane}}
\subsubsection{Failure to stop and remain stopped for pedestrian (ORS 811.028)}

\begin{center}
    $\lnot EGO.isDeceleration \wedge (on(pedestrian, EGO.predLane) \vee on(pedestrian, adjLane(EGO.predLane) \vee disTo(pedestrian, EGO.predLane)) $
\end{center}

\subsubsection{Failure to drive on right (ORS 811.295)}
\begin{center}
    $ (rmnWdAhd > 2 \cdot EGO.width) \wedge onLft(EGO, centLine) \wedge \lnot (isPassing \vee (turnDec = left) \vee hasObsAhd \vee numLane >= 3) $
\end{center}

\noindent\underline{\textbf{Speed limit violations}}

\subsubsection{Violating a speed limit (ORS 811.111)}

\begin{center}
    $ EGO.isAccelration \wedge (rdTyp = highway) \wedge (EGO.spd > spdLim)$
\end{center} 

\subsubsection{Violation of basic speed rule (ORS 811.100)}

\begin{center}
    $ EGO.isAccelration \wedge (rdTyp = highway) \wedge (EGO.spd > adptSpdLim(trf, env))$
\end{center}

\subsection{Deceleration Violations (Deceleration)}

\subsubsection{Impeding traffic (ORS 811.130)}

\begin{center}
    $ EGO.isDeceleration \wedge (\sum\Delta NPCBack.pos < \theta_1) $
\end{center}

\subsubsection{Unlawful stop or deceleration (ORS 811.500)}

\begin{center}
    $ (EGO.isDeceleration \vee EGO.isStopping \vee (\Delta EGO.brk < \theta_2)) \wedge (\lnot EGO.EGO.brkSig) $
\end{center}

\subsection{Other Violation}

\subsubsection{Reckless driving (ORS 811.140) (?)}

\subsubsection{Careless driving (ORS 811.135) (?)}

\subsubsection{Misuse of special left turn lane (ORS 811.346)}
\begin{center}
    $on(EGO, specLftLane) \wedge (turnDecision \neq left)$
\end{center}

==> table/car_status.tex <==
\begin{table*}[!t]
\centering
\caption{Car status variables}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Variable}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Description}}       & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Example}} \\ \midrule
brkSig                                                    & Bool                                                       & True if ego's brake signal is turned on                                 & True / False                                                 \\
turnSig                                                     & Enum                                                       & Return whether left signal or right signal is turned on or none of them & none, left, right                                            \\
width                                                          & Double                                                     & Ego's Width                                                             & 2 (m)                                                        \\
dir                                                            & Vector                                                     & The direction of car's head, from center to head      & (1, 1, 1)                                                    \\
sigDur                                                         & Double                                                     & The distance that the ego's signals are continuously turned on          & 30 (m)                                                       \\
spdLim                                                         & Double                                                     & Ego's speed limit                                                       & 40 (km/h)                                                    \\ \bottomrule
\end{tabular}
\end{table*}

==> table/driving_status.tex <==
\begin{table*}[!t]
\centering
\caption{Driving status variables}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Variable}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Description}} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Example}} \\ \midrule
spd                                                          & Double                                                     & Ego's driving speed                                               & 40 (km/h)                                                    \\
brk                                                          & Double                                                     & Ego's brake percentage                                            & 40 (\%)                                                      \\
acc                                                          & Double                                                     & Ego's acceleration                                            & 40 (m/$s^2$)                                                      \\
pos                                                          & Vector                                                     & Ego's position                                            & (1, 1, 1)                                                   \\
moveDir                                                          & Vector                                                     & Ego's moving direction                                        & (1, 1, 1)                                                \\
predLane                                                       & Lane                                                       & Predicted lane that ego is approaching in next 3 seconds          & Lane(id, direction, v.v)                                     \\
turnDec                                                        & Enum                                                       & Ego's turning decision                                            & none, left, right                                            \\
hasClrView                                                  & Bool                                                       & True if ego has a clear view when enters a lane or roadway        & True / False                                                 \\
isBacking                                                      & Bool                                                       & True if ego is backing                                            & True / False                                                 \\
isCruising                                                     & Bool                                                       & True if ego is cruising                                           & True / False                                                 \\
isPassing                                                      & Bool                                                       & True if ego is passing other vehicles                             & True / False                                                 \\
isAccelerating                                                 & Bool                                                       & True if ego is accelerating                                       & True / False                                                 \\
isSteadyDriving                                                & Bool                                                       & True if ego is driving steadily                                       & True / False                                                 \\
isDecelerating                                                 & Bool                                                       & True if ego is decelerating                                       & True / False                                                 \\
isDirectionChanging                                            & Bool                                                       & True if ego is changing it's direction                                       & True / False                                                 \\
isStopping                                                     & Bool                                                       & True if ego is stopping                                           & True / False                                                 \\
isTurning                                                     & Bool                                                       & True if ego is turning                                           & True / False                                                 \\
isLaneChanging                                                 & Bool                                                       & True if ego is changing into other lane                           & True / False                                                 \\ \bottomrule
\end{tabular}
\end{table*}

==> table/driving_status_backup.tex <==
\begin{table*}[]
\centering
% \footnotesize
\caption{Driving status variables in \tool}\label{tab:driving-status}
\begin{tabular}{l|c|c|l}
\toprule
\multicolumn{1}{c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Symbol}} & \multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c}{\textbf{Remarks}} 
\\ \midrule 
ego\_pos   & $P_{ego}$                & Vector                                     & The ego vehicle's position (Easting and Northing)                                                      
\\ \midrule
ego\_past\_pos   & ${P}^{past}_{ego}$                & Vector                                     & The previous position of ego vehicle                                                          
\\ \midrule
ego\_predict\_pos   & $\tilde{P}_{ego}$                & Vector                                     & The predicted ego vehicle's position (Easting and Northing)                                                             
\\ \midrule
ego\_speed  & $v_{ego}$               & Number                                                                                     & Speed of ego vehicle (m/s)                    \\ \midrule
ego\_acc & $a_{ego}$ &  Number & Accelaration of ego vehicle (m/$s^2$)
\\ \midrule
ego\_velocity & $\overrightarrow{v_{ego}}$ &  Vector & Velocity of ego vehicle
\\ \midrule
ego\_brake & $brake_{ego}$ &  Number & Braking percentage of ego vehicle (\%)
\\ \midrule
ego\_past\_brake & $brake^{past}_{ego}$ &  Number & Past braking percentage of ego vehicle (\%)
\\ \midrule
ego\_trajectory & $ line_{ego}$ &  Vector & The coefficients k, b of the line between $P_{ego}$  and $\tilde{P}_{ego}$  
\\ \midrule
npc\_pos   & $P_{npc}$                & Vector                                     & The NPC's position (Easting and Northing)                                                                      
\\ \midrule
npc\_predict\_pos   & $\tilde{P}_{npc}$                & Vector                                     & Predicted position of NPC                                   \\ \midrule  
npc\_speed  & $v_{npc}$     & Number                                      & Speed of NPC (m/s)
\\ \midrule
npc\_acc & $a_{npc}$ &  Number & Accelaration of NPC (m/$s^2$)
\\ \midrule
npc\_velocity & $\overrightarrow{v_{npc}}$ &  Vector & Velocity of NPC
\\ \midrule
npc\_trajectory & $ line_{npc}$ & Vector & The coefficients k, b of the line between $P_{npc}$  and $\tilde{P}_{npc}$ 
\\ \bottomrule

\end{tabular}
\end{table*}

==> table/dynamic_objects_status_backup.tex <==
\begin{table*}[]
\centering
% \footnotesize
\caption{Status variables of the NPC vehicle and pedestrian in \tool}\label{tab:dynamic-obj-status}
\begin{tabular}{l|c|c|l}
\toprule
\multicolumn{1}{c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Symbol}} & \multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c}{\textbf{Remarks}} 
\\ \midrule 

obj\_pos   & $P_{obj}$                & Vector                                     & The position (Easting and Northing) of the NPC vehicle or pedestrian                                                                      
\\ \midrule
obj\_predict\_pos   & $\tilde{P}_{obj}$                & Vector                                     & Predicted position of the NPC vehicle or pedestrian                                  \\ \midrule  
obj\_speed  & $v_{obj}$     & Number                                      & Speed of NPC or pedestrian (m/s)
\\ \midrule
obj\_acc & $a_{obj}$ &  Number & Accelaration of NPC or pedestrian (m/$s^2$)
\\ \midrule
obj\_velocity & $\overrightarrow{v_{obj}}$ &  Vector & Velocity of NPC or pedestrian
\\ \midrule
obj\_trajectory & $ line_{obj}$ & Vector & The coefficients k, b of the line between $P_{obj}$  and $\tilde{P}_{obj}$ 
\\ \bottomrule

\end{tabular}
\end{table*}

==> table/ego_status_backup.tex <==
\begin{table*}[]
\centering
% \footnotesize
\caption{Driving status variables of the ego vehicle in \tool}\label{tab:ego-status}
\begin{tabular}{l|c|c|l}
\toprule
\multicolumn{1}{c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Symbol}} & \multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c}{\textbf{Remarks}} 
\\ \midrule 
ego\_pos   & $P_{ego}$                & Vector                                     & The ego vehicle's position (Easting and Northing)                                                      
\\ \midrule
ego\_past\_pos   & ${P}^{past}_{ego}$                & Vector                                     & The previous position of ego vehicle                                                          
\\ \midrule
ego\_predict\_pos   & $\tilde{P}_{ego}$                & Vector                                     & The predicted ego vehicle's position (Easting and Northing)                                                             
\\ \midrule
ego\_speed  & $v_{ego}$               & Number                                                                                     & Speed of ego vehicle (m/s)                    \\ \midrule
ego\_acc & $a_{ego}$ &  Number & Accelaration of ego vehicle (m/$s^2$)
\\ \midrule
ego\_velocity & $\overrightarrow{v_{ego}}$ &  Vector & Velocity of ego vehicle
\\ \midrule
ego\_brake & $brake_{ego}$ &  Number & Braking percentage of ego vehicle (\%)
\\ \midrule
ego\_past\_brake & $brake^{past}_{ego}$ &  Number & Past braking percentage of ego vehicle (\%)
\\ \midrule
ego\_trajectory & $ line_{ego}$ &  Vector & The coefficients k, b of the line between $P_{ego}$  and $\tilde{P}_{ego}$  

\\ \bottomrule

\end{tabular}
\end{table*}

==> table/environment_status.tex <==
\begin{table*}[!t]
\centering
\caption{Environment status variables}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Variable}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Description}} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Example}} \\ \midrule
env                                                           & Environment                                                     & Environtment around EGO                                                       & Environment(time, weather)                                                   \\
time                                                           & Double                                                     & Time of day                                                       & 10, 14, 20                                                   \\
weather                                                            & Weather                                                       & Weather status includes fog, rain and wetness level                                                         & Weather(fog, rain, wetness)                     
                              \\ \bottomrule
\end{tabular}
\end{table*}

==> table/road_status.tex <==
\begin{table*}[!t]
\centering
\caption{Road status variables}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Variable}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Description}}    & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Example}} \\ \midrule
spdLim                                                     & Double                                                     & Road's speed limit                                                   & 65 (km/h)                                                    \\
rdTyp                                                       & Enum                                                       & Type of road                                                         & highway, two\_way, divided\_highway                          \\
centLine                                                     & Line                                                       & The centerLine of a road                                             & Line(type, equation)                                         \\
rmnWdAhd                                            & Double                                                     & The width of the remaining space in front of the vehicle & 5 (m)                                                        \\
numLane                                                        & Int                                                        & Number of lanes in road                                              & 5                                                            \\
curLane                                                    & Lane                                                       & The lane that the EGO is traveling in                                & Lane(id, position, direction, v.v)                           \\
motorLane                                                      & Lane                                                       & The lane permitting motor driving on                                 & Lane(id, position, direction, v.v)                           \\
rightCurb                                                      & Line                                                       & The right-most curb of a road                                        & Line(type, equation)                                         \\
specLftLane                                            & Lane                                                       & The lane specifically designed for left-turning vehicles             & Lane(id, position, direction, v.v)                           \\
extmLftLane                                                & Lane                                                       & The lane on the far left side of the road                            & Lane(id, position, direction, v.v)                           \\
extmRgtLane                                               & Lane                                                       & The lane on the far right side of the road                           & Lane(id, position, direction, v.v)                           \\
sftyZone                                                     & SpecialZone                                                & Safety Zone, the place specifically designed for pedestrian to stand      & SpecialZone(position, size)                                  \\
rotTrfIsl                                            & SpecialZone                                                & Rotary Traffic Island, a circular area lies on the center of a roundabout                   & SpecialZone(position, size)                                  \\
bicTrail                                                   & SpecialZone                                                & BicycleTrail, The lane designed to allow cyclists to drive on                      & SpecialZone(position, size)                                  \\
inter                                                      & SpecialZone                                                & A normal intersection                                                & SpecialZone(position, size)                                  \\
swkAhd                                                  & SpecialZone                                                & The sidewalk area in front of EGO                                    & SpecialZone(position, size)                                  \\
rndabt                                                     & SpecialZone                                                & A normal roundabout                                                  & SpecialZone(position, size)                                  \\
npZone                                                  & SpecialZone                                                & No Passing Zone, A place is not allowed a vehicle to pass another vehicle             & SpecialZone(position, size)                                  \\
t\_inter                                                       & SpecialZone                                                & A T-shape intersection                                               & SpecialZone(position, size)                                  \\
hasCrwkAhd                                              & Bool                                                       & True if there is a crosswalk area in front of EGO                    & True / False                                                 \\
hasObsAhd                                              & Bool                                                       & True if there are some obstacles in front of EGO                     & True / False                                                 \\ \bottomrule
\end{tabular}
\end{table*}

==> table/road_status_backup.tex <==
\begin{table*}[]
\centering
% \footnotesize
\caption{Road status variables in \tool}\label{tab:road-status}
\begin{tabular}{l|c|c|l}
\toprule
\multicolumn{1}{c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Symbol}} & \multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c}{\textbf{Remarks}} 
\\ \midrule 
intersect\_position   & $\tilde{P}_{I}$                & Vector                                     & Predicted collising point of ego and npc                                                         
\\ \midrule
lane\_direction  & $\overrightarrow{d_{lane}}$               & Vector                                                                                     & Direction of lane ego located                   \\ \midrule
lane\_id & $id_{lane}$ &  Number & Lane ID ego located \\ \midrule
next\_lane\_direction & $\overrightarrow{d_{\widetilde{lane}}}$ &  Vector & Direction of lane ego located in next 3 seconds 
\\ \midrule
next\_lane\_id & $id_{\widetilde{lane}}$ &  Number & Lane ID ego located in next 3 second
\\ \midrule
traffic\_light\_color & $light_{status}$ &  Number & The nearest traffic light color
\\ \midrule
stop\_line & $stop\_line()$ &  Function & \makecell{The value when substituting point into the equation of \\ the traffic stop line}
\\ \midrule
speed\_limit & $speed_{limit}$ & Number & The allowance speed limit of the road (m/s)
\\ \bottomrule

\end{tabular}
\end{table*}

==> table/traffic_signal_status.tex <==
\begin{table*}[!t]
\centering
\caption{Traffic signal status variables}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Variable}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Description}}                         & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Example}} \\ \midrule
uTurnSig                                                    & TrafficSignal                                              & The signal shows that vehicles is permitted to perform an U-turn                          & TrafficSignal(position, type, v.v)                           \\ 
trfLig                                                   & TrafficSignal                                              & The devices used to control the flow of traffic at intersections, v.v & TrafficSignal(position, type, v.v)                           \\ 
stopSign    & TrafficSignal &   The sign indicates that vehicles must come to a complete stop   &   TrafficSignal(position, type, v.v)                           \\ \bottomrule
\end{tabular}
\end{table*}

==> table/traffic_status.tex <==
\begin{table*}[!t]
\centering
\caption{Traffic status variables}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Variable}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Description}} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Example}} \\ \midrule
trf                                       & Traffic                                                       & Traffic status around EGO                          & Traffic(npc, pedestrian, bicyclist, v.v)                                                 \\
freeOfTrf                                       & Bool                                                       & True if EGO is free of oncomming traffic                          & True / False                                                 \\
NPC                                                            & NPCVehicle                                                 & The npc vehicles driving around the EGO                        & NPCVehicle(position, direction, v.v)                         \\
NPCBack                                                        & NPCVehicle                                                 & The npc vehicles driving behind the EGO                        & NPCVehicle(position, direction, v.v)                         \\
NPCAhd                                                       & NPCVehicle                                                 & The npc vehicles driving in front of the EGO                   & NPCVehicle(position, direction, v.v)                         \\
NPCOppo                                                       & NPCVehicle                                                 & The npc vehicles driving in opposite direction                   & NPCVehicle(position, direction, v.v)                         \\
bicAhd                                                 & NPCVehicle                                                 & The bicyclists riding in front of the EGO                      & NPCVehicle(position, direction, v.v)                         \\
pedesAhd                                                & Pedestrian                                                 & The pedestrians walking in front of the EGO                    & Pedestrian(position, direction, v.v)                         \\ \bottomrule
\end{tabular}
\end{table*}

==> table/utility_function.tex <==
\begin{table*}[!t]
\centering
\caption{Utility Function}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l }
\toprule
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Function}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Return Type}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Definition}}   \\ \midrule
isInter(vehicle, line)                                     & Lane                                                              & True if a vehicle intersects with a line (Lane Boundary)           \\
disTo(object, object)                                          & Bool                                                              & Distance from a vehicle to another one                             \\
on(vehicle, object)                                            & Bool                                                              & True if vehicle is on this object (or special zones)               \\
adjLane(lane)                                             & Double                                                            & Adjacent lane                                                      \\
yldDec(vehicle)                                         & Bool                                                              & True if a vehicle decides to yield the right of way to another one \\
onLft(vehicle, object)                                        & Lane                                                              & True if vehicle is on the left of object                           \\
onRgt(vehicle, object)                                       & Bool                                                              & True if vehicle is on the right of object                          \\
aprc(vehicle, vehicle)                                     & Bool                                                              & True if a vehicle is approaching another one                       \\
angle(vector, vector)                                     & Double                                                              & The angle created by two vector                      \\
adptSpdLim(trf, env)                                     & Double                                                              & The road's speed limit in specific traffic, weather, v.v                      \\
hasClrView(lane)                                            & Bool                                                              & True if EGO has a clear view on specific lane                      \\ \bottomrule
\end{tabular}
\end{table*}

==> violations/acceleration.tex <==
\subsection{Dangerous acceleration}


Acceleration is the rate of increasing the vehicle's speed.
\begin{center}
    $ isAcceleration = acc \geq \theta_4 $
\end{center}


Dangerous acceleration is the increase in speed that could cause the AV to result in loss of control or inability to react safely to surrounding conditions and obstacles. 
In practice, determining whether an acceleration is dangerous depends on various factors such as road conditions, weather conditions, traffic density, etc. Without loss of generality, we consider an acceleration as dangerous if it either (i) increases the speed to exceed the safe limits or (ii) leads the ego to be too close to the other obstacle(s). 
% In addition, the acceleration is considered too fast if the acceleration value is greater than a pre-defined threshold. For example, on public road, acceleration from 0 to 100km/h in under 6 seconds is considered aggressive and dangerous~\cite{}. 

For (i), operating the ego vehicle at a high speed reduces its reaction time to unexpected events.
Additionally, ADSs rely on multiple sensors, such as LIDAR, radar, and cameras. At high speeds, the effectiveness of these sensors could be decreased, significantly affecting the system's response time to obstacles, road signs, and environmental changes. This reduction in sensor performance could increase the risk of accidents.
Moreover, the speed limit is a traffic rule that not only human drivers but also the ADSs must obey. Therefore, to ensure safety, if the ADS accelerates beyond the allowable speed, $Speed_{limit}$,  which is dynamically determined according to the road on which the ego is driving, the ADS violates the safety condition of dangerous acceleration.

\begin{equation}
\label{eq:speed_limit}
v_{ego} > Speed_{limit}
\end{equation}
%

For (ii), besides maintaining a safe speed, ADSs must also maintain an appropriate distance from the other obstacles while traveling. If the ego vehicle gets too close to an obstacle, it has less time to detect and process the information. This could potentially fail to take correct action. 
Thus, dangerous acceleration is also defined as acceleration that leads the ego vehicle to be too close to an obstacle, and their trajectories could intersect. 
Note that an obstacle could be a dynamic object, e.g., NPC vehicle or pedestrian, or a static object, e.g., sidewalks.


\begin{equation}
\label{eq:acc_collision}
\begin{array}{l}

\begin{cases}
(v_{ego} > \theta_{speed}) \, \wedge  \, (a_{ego} > 0)\\
CD \leq SD\\
line_{ego} \cap line_{obj} \neq \emptyset
\end{cases}
\end{array}
\end{equation}

In Condition~\ref{eq:acc_collision}, the first sub-condition specifies that the ego vehicle is accelerating, with both its speed and acceleration rate being greater than 0. The second sub-condition indicates that the ego vehicle is too close to the obstacle when the current distance (CD) between them is smaller than the safety distance (SD). The detail of calculating safety distance is presented in Sec.~\ref{?}. The last sub-condition illustrates a possible collision since the trajectories of the ego vehicle and the obstacle intersect.

In summary, \tool considers that the ADS violates the dangerous acceleration if either Condition~(\ref{eq:speed_limit}) or Condition~(\ref{eq:acc_collision}) is satisfied.



==> violations/backing.tex <==
\subsection{Backing}
\begin{center}
    $ isBacking = isDirectionChanging \wedge (EGO.dir \cdot EGO.moveDir) < 0 $
\end{center}


==> violations/cruising.tex <==
\subsection{Cruising}

\begin{center}
    $ isCruising = isSteadyDriving $
\end{center}

==> violations/deceleration.tex <==
\subsection{Sudden deceleration}

% \begin{equation}
% \label{eq:brake_threshold}
% brake_{ego} > \theta_{brake}
% \end{equation}

% \begin{equation}
% \label{eq:dec_collision}
% \begin{array}{l}

% \begin{cases}
% brake_{ego} > 0\\
% CD \leq SD\\
% line_{ego} \cap line_{obj} \neq \emptyset
% \end{cases}
% \end{array}
% \end{equation}


\begin{center}
    $ isDeceleration = acc \leq -\theta_4 $
\end{center}

==> violations/general.tex <==


% Ensuring that autonomous vehicles (AVs) to operate reliably on real-world roads without violating the safety conditions is utmost important. Compliance with the safety conditions during operating on road not only reduces the risks of accidents but also improve the traffic flow and enhance the moving comfort for passengers. Therefore, rigorously testing the ADSs under diverse simulation scenarios is essential to prevent any violations of the safety conditions. 

In practice, to travel from the entry to the destination, ADSs rely on three basic driving behaviors, including \textit{acceleration}, \textit{deceleration}, and \textit{direction changing}. If these behaviors are exhibited improperly, the ADSs may fail to maintain the safety conditions, which could cause discomfort traveling for passengers and could even dangerously result in an accident. In this work, we focus on testing the ability of ADSs in controlling these behaviors safely and reliably.

First, \textit{acceleration} is the rate at which vehicle increases speed. If the speed is dangerously increased to significantly higher than the speed limit, this speeding-up behavior becomes hazardous. Indeed, high speed not only make the vehicle control more challenging, but also increase the damage severity if the accidents happens. Therefore, one of the safety conditions that must be maintained is to avoid \textit{dangerous acceleration}.

Second, \textit{deceleration} is the reduction in the vehicle's speed. Depending on the traffic flow and the road conditions, vehicles could need to slow down to ensure safety. However, if the deceleration occurs rapidly and suddenly, it could cause the wheels to lock up, leading to skidding and loss of steering control. Sudden deceleration could also increase the risk of rear-end collisions or chain-reaction crashes. Therefore, another safety condition need to maintain to not violate is \textit{sudden deceleration}.

Third, \textit{direction changing} is the capability of an ADS to alter its course or path in responding to driving conditions, avoiding obstacles, or making navigation. This ability allows ADSs to smoothly perform necessary maneuvers such as turning at intersections, changing lanes, or overtaking other vehicles. However, if these maneuvers are improperly executed, they could pose dangers for both the AVs and the surrounding vehicles or pedestrians. For example, improper turn is one of the top 25 causes of car accidents~\cite{top25causes}. Therefore, it is critical to ensure the safety conditions related to direction changing, including avoiding \textit{improper turns}, \textit{improper lane changing}, and \textit{improper overtaking}.


In this paper, \tool aims to generate safety critical scenarios to find the violations of ADSs in aforementioned safety conditions. According to the fundamental driving behaviors of a vehicle on road, i.e., acceleration, deceleration, direction changing, we categorize the safety conditions which ADSs should not violate into 5 groups.  They are dangerous acceleration, sudden deceleration, improper turn, improper lane changing, and improper overtaking.


% \input{table/ego_status}
% \input{table/dynamic_objects_status}
% \input{table/road_status}

% Table~\ref{tab:ego-status}, Table~\ref{tab:dynamic-obj-status}, and Table~\ref{tab:road-status} define the necessary variables which used for formulating the safety conditions. Specifically, Table~\ref{tab:ego-status} defines the variables used to describe properties of the ego. 
% The status of the dynamic objects, such as NPC vehicles and the pedestrians, are illustrated in Table~\ref{tab:dynamic-obj-status}.
% The road status variables are defined in Table~\ref{tab:road-status}, which contains variables used for describing the properties of the road which the AV is currently driving on. 

==> violations/lane_changing.tex <==
\subsection{Improper lane changing}

\begin{center}
    $ isDirectionChanging = angle(EGO.moveDir, curLane.dir) > \theta_5 $
\end{center}

\begin{center}
    $ isLaneChanging = isDirectionChanging \wedge angle(curLane.dir, EGO.predLane.dir) \leq \theta_6 $
\end{center}


==> violations/overtaking.tex <==
\subsection{Improper overtaking}

\begin{center}
    $ isPassing = isAcceleration \wedge (EGO.moveDir \cdot NPCAhd.moveDir > 0) \wedge (EGO.spd > NPCAhd.spd) $
\end{center}

==> violations/steady_driving.tex <==
\subsection{Steady Driving}

\begin{center}
    $ isSteadyDriving = acc \in \left ( -\theta_4, \theta_4 \right ) $
\end{center}


==> violations/stopping.tex <==
\begin{center}
    $ isStopping = (EGO.spd \approx 0) $
\end{center}


==> violations/turn.tex <==
\subsection{Improper turn}

\begin{center}
    $ isTurning = isDirectionChanging  \wedge angle(curLane.dir, EGO.predLane.dir) > \theta_6 $
\end{center}
